Navigation In Urban Environments Amongst Pedestrians Using Multi-Objective Deep Reinforcement Learning

Urban autonomous driving in the presence of pedestrians as vulnerable road users is still a challenging and less examined research problem. This work formulates navigation in urban environments as a multi objective reinforcement learning problem. A deep learning variant of thresholded lexicographic Q-learning is presented for autonomous navigation amongst pedestrians. The multi objective DQN agent is trained on a custom urban environment developed in CARLA simulator. The proposed method is evaluated by comparing it with a single objective DQN variant on known and unknown environments. Evaluation results show that the proposed method outperforms the single objective DQN variant with respect to all aspects.

==> background_copy.tex <==
\section{BACKGROUND}
\subsection{Single Objective Reinforcement Learning}
Reinforcement learning (RL) is often formulated as a Markov Decision Process (MDP), a tuple \textit{(S, A, T, R)}, characterized by a set of states \textit{S}, a set of actions \textit{A} and a scalar reward function \textit{R} and a transition function \textit{T}. 
In the single-objective reinforcement learning (SORL), 
at each time \textit{t}, an agent interacts with the environment by observing the state \textit{s\textsubscript{t}} and performing an action \textit{a\textsubscript{t}}, according to some policy $\pi$. Performing an action generates a reward \textit{r\textsubscript{t}} and takes the agent to next state \textit{s\textsubscript{t+1}} and the process repeats until a termination condition.
The agents goal is to maximize the expected discounted
reward $R_{t} = \sum_{t=0}^{T} \gamma \cdot r_{t}$, where $\gamma \in [0, 1]$ is a discount factor deciding the importance of future rewards.

In Q-learning algorithm, actions are selected using a Q-function \textit{Q(s,a)}, 
which constitutes the expected discounted reward for executing an
action \textit{a} in state \textit{s}.
The optimal action for a state \textit{s} is defined as:
\begin{equation}
    a_{}{'} = \underset{a \in A}{\arg\max}\:Q(s, a) 
\end{equation}
An agent is said to be following an optimal policy $\pi^{*}$, given it always selects the optimal action. The function \textit{Q(s,a)} helps in forming an optimal policy by simply selecting actions with highest Q-values.

In Deep Q-Networks, the \textit{Q(s,a)} values are approximated using deep neural networks  making Q-learning feasible for many real-world complex applications.
A variant of DQN, called Double Deep Q-Network (DDQN) uses a separate target network to make the learning process more stable. Its parameters are periodically updated using action network.

\subsection{Multi-Objective Reinforcement Learning}
In several complex applications there exist more than one objective to be considered.
If these objectives are independent or directly related, they could be merged to form a single objective. However, often the objectives are in conflict, that is, maximizing one objective causes minimization of another.
For such applications, Multi-Objective Reinforcement Learning (MORL) is used to characterize two or more objectives simultaneously.
MORL is often modelled as Multi-objective Markov Decision Process (MOMDP) instead of single objective MDP.
An MORL agent, instead of a single reward, receives a vector of rewards at each time step, corresponding to each objective. 
Given \textit{O} as a set of \textit{n} objectives, the reward vector is defined as: \textit{R = [r\textsubscript{1}, r\textsubscript{2}, .. , r\textsubscript{n}]}, where \textit{r\textsubscript{i}} represents scalar reward for objective \textit{o\textsubscript{i}}$\in$\textit{O}.
The expected discounted reward for an objective \textit{o\textsubscript{i}}, at time \textit{t}, is defined as:
\begin{equation}
    R_{i,t} = \sum_{t=0}^{T} \gamma \cdot r_{i,t}
\end{equation}
Usually, a separate Q-function $Q_{i}(s,a)$ is considered for each objective such that:
\begin{equation}
    Q_{i}(s,a) = E [R_{i,t}|s_{t} = s, a_{t} = a]
\end{equation}
resulting into a vector of Q-functions.
At each time step \textit{t}, the agent uses the function \textit{Q\textsubscript{i}(s,a)} to find the optimal action satisfying objective \textit{q\textsubscript{i}}.
Since the agent can perform a single action at a time, a method to find this single action 
is required.





\subsection{Thresholded Lexicographic Q-learning}
Threshold lexicographic Q-Learning (TLQ-Learning), introduced by \textit{Gabor et al.} \cite{} is an algorithm which uses lexicographic ordering on objectives based on their priorities.
A threshold $\tau_{i}$ is used for each objective to define the minimum or
maximum acceptable Q-value (depending on whether the objective is
to be minimised or maximised).
Thresholds are set to the first $i-1$ objectives and the last objective
is left unconstrained.

Selection of action is done by using a combination of thresholding and lexicographic ordering to the objective's Q-values \cite{}. 
If \textit{Q\textsubscript{s,a,i}} is the value for \textit{i\textsuperscript{th}} objective corresponding to action \textit{a} in state \textit{s} and \textit{T\textsubscript{i}} is threshold, then:
\begin{equation}
    CQ_{s,a,i} = min(Q_{s,a,i}, C_{i})
\end{equation}
Given a state \textit{s}, a greedy action \textit{a\textsuperscript{'}} is selected satisfying the recursive function as defined below:
\input{tlo_algorithm}










==> method_copy.tex <==












==> tlo_algorithm_copy.tex <==
\begin{algorithm}
\caption{Superior}
\SetKwInput{KwInput}{Input}                %
\SetKwInput{KwOutput}{Output}              %
\DontPrintSemicolon
  
  \KwInput{vector value \textit{TQ(s,a)}, \textit{TQ(s,a)}, }
  \KwOutput{Your output}
  \KwData{Testing set $x$}

  \SetKwFunction{FMain}{Main}
  \SetKwFunction{FSum}{Sum}
  \SetKwFunction{FSub}{Sub}
  \SetKwFunction{FSuperior}{Superior}
 
  \SetKwProg{Fn}{}{:}{}
  \Fn{\FSuperior{$TQ_{s,a^{'}}$, $TQ_{s,a}$, i}}{
        \textbf{if} $TQ_{s,a^{'}} > TQ_{s,a}$  \;
            \KwRet True\;
        \textbf{else if} $TQ_{s,a^{'}} = TQ_{s,a}$ \;
            \KwRet True\;
  }
  \;

\end{algorithm}





\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

    \Input{$TQ_{s,a^{'}}$, $TQ_{s,a}$, \textit{i}}
    \Output{if $TQ_{s,a}$ superior to $TQ_{s,a^{'}}$}
    
    \uIf{$TQ_{s,a^{'},i} > TQ_{s,a,i}$}
    {
        \textbf{return} true\;
    }
    \uElseIf{$TQ_{s,a^{'},i} = TQ_{s,a,i}$}
    {
        \uIf{i = n}
        {
            \textbf{return} true
        }
        \Else
        {
            \textbf{return} Superior($TQ_{s,a^{'}}$,$TQ_{s,a}$, $i+1$)    
        }
    }
    \Else
    {
        \textbf{return} false
    }
    \caption{Superior}
\end{algorithm}
$TQ_{s,a^{'}}$, $TQ_{s,a}$, i
